Augmented Reality and Robotics: A Survey and Taxonomy for AR-enhanced Human-Robot Interaction and Robotic Interfaces

This paper contributes to a taxonomy of augmented reality and robotics based on a survey of 460 research papers. Augmented and mixed reality (AR/MR) have emerged as a new way to enhance human-robot interaction (HRI) and robotic interfaces (e.g., actuated and shape-changing interfaces). Recently, an increasing number of studies in HCI, HRI, and robotics have demonstrated how AR enables better interactions between people and robots. However, often research remains focused on individual explorations and key design strategies, and research questions are rarely analyzed systematically. In this paper, we synthesize and categorize this research field in the following dimensions: 1) approaches to augmenting reality; 2) characteristics of robots; 3) purposes and benefits; 4) classification of presented information; 5) design components and strategies for visual augmentation; 6) interaction techniques and modalities; 7) application domains; and 8) evaluation strategies. We formulate key challenges and opportunities to guide and inform future research in AR and robotics.

==> revision-summary.tex <==
MAIN ISSUES IDENTIFIED, WITH REFERENCES TO REVIEWS:
-The dataset and the inclusion criteria (R1, R3):
Revise the selection criteria, which appear currently broad (R1, R3); improve the
coverage of the dataset and make the selection process more reproducible (R1)

- The taxonomy and the analysis of the literature (R1, 2AC):
Improve the discussion of the taxonomy dimensions and of the work cited, also
providing summaries of the findings (i.e. on benefits/drawbacks uncovered by the
analysed papers), where the surveyed papers fit into the taxonomy and whether
patterns emerge or there are evident gaps, see both R1 and 2AC. Discuss the
interrelationships between the taxonomy dimensions (R1).

- Challenges and conclusions (R1, R3, 2AC):
More clearly derive the identified challenges and opportunities for future
research directions from the analysis of the surveyed papers by making more
explicit connections (R1, 2AC); provide deeper insights and more forward-looking
conclusions and takeaway messages (R1, R3, 2AC).

- Missing details and unclear points (2AC, R1):
Clarify the missing details and the unclear points highlighted in the individual
reviews of 2AC and R1;

- Further aspects (2AC, R1):
Address issues with figures (2AC, R1), and references and spelling (2AC)
